Verifiable Homomorphic Linear Combinations in Multi-Instance Time-Lock Puzzles

Time-Lock Puzzles (TLPs) have been developed to securely transmit sensitive information into the future without relying on a trusted third party. Multi-instance TLP is a scalable variant of TLP that enables a server to efficiently find solutions to different puzzles provided by a client at once. Nevertheless, existing multi-instance TLPs lack support for (verifiable) homomorphic computation. To address this limitation, we introduce the "Multi-Instance partially Homomorphic TLP" (MH-TLP), a multi-instance TLP supporting efficient verifiable homomorphic linear combinations of puzzles belonging to a client. It ensures anyone can verify the correctness of computations and solutions. Building on MH-TLP, we further propose the "Multi-instance Multi-client verifiable partially Homomorphic TLP" (MMH-TLP). It not only supports all the features of MH-TLP but also allows for verifiable homomorphic linear combinations of puzzles from different clients. Our schemes refrain from using asymmetric-key cryptography for verification and, unlike most homomorphic TLPs, do not require a trusted third party. A comprehensive cost analysis demonstrates that our schemes scale linearly with the number of clients and puzzles.

==> VH-TLP--proof.tex <==
%!TEX root = main.tex





\section{Proof of Theorem \ref{theo:security-of-VH-TLP}}\label{sec::VH-TLP-proof}

 
In this section, we prove the security of \tf, i.e., Theorem \ref{theo:security-of-VH-TLP}. 



\begin{proof}


%%%%%
In the proof of Theorem \ref{theo:security-of-VH-TLP}, we consider a strong adversary that \textit{always corrupts} \srv and some clients. Thus, the proof considers the case where corrupt  \srv learns the secret inputs, secret parameters, and the messages that corrupt clients receive from honest clients. The messages that an adversary \adv receives are as follows.

\begin{itemize}[label=$\bullet$]
 \item by the end of the puzzle generation phase, it learns:
 %
  $$Set_{\st 1}=\Big\{\mxsqr, \{ N_{\st \prt}, \Delta_{\st \prt}, T_{\st \prt},  r_{\st \prt}, com_{\st \prt}, \vec{o}_{\st \prt}\}_{\st \forall \prt, 1\leq \prt \leq n}, \{K_{\st j}\}_{\st \forall \advb_{\st j}\in \corupt}
 %
 \Big\}$$
 
  where $\corupt$ is a set of corrupt parties, including server \srv.  
 
 
 \item by the end of the linear combination phase (before any puzzle is fully solved), it also learns:  
 %
 $$Set_{\st 2}=\Big\{ trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}, Y,  \{g_{\st 1}, \ldots, g_{\st \bar{t}}\}, \{com'_{\st \prt}, h_{\st \prt}, d_{\st 1, \prt},\ldots, d_{\st \bar{t}, \prt}   \}_{{ \st \forall \prt, 1\leq \prt \leq n}}, \{\bar f_{\st {\st l}}, \vv{ \gamma}'_{\st{l}}\}_{\st \forall\cl_{l}\in \{\corupt\cap\idx\}}\Big\}$$
 
  where $trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}$ is a set of messages sent to \srv during the execution of $\ole^{\st +}$. 
 \end{itemize}


%%%%%%
We initially prove that \tf is privacy-preserving, w.r.t. Definition \ref{def:privacy-vh-tlp}. 


\begin{lemma}\label{lemma:VH-TLP-privacy}
If the sequential modular squaring assumption holds, factoring $N$ is a hard problem, \prf is secure,  $\ole^{\st +}$ is secure (i.e., privacy-preserving), and the commitment scheme satisfies the hiding property, then \tf is privacy-preserving, w.r.t. Definition \ref{def:privacy-vh-tlp}. 

\end{lemma}

\begin{proof}
%In the proof of Lemma \ref{lemma:VH-TLP-privacy}, we consider a strong adversary that \textit{always corrupts} \srv and some clients. Thus, the proof considers the case where corrupt  \srv learns the secret inputs, secret parameters, and the messages that corrupt clients receive from honest clients. The messages that an adversary \adv receives are as follows.
%
%\begin{itemize}[label=$\bullet$]
% \item by the end of the puzzle generation phase, it learns:
% %
%  $$Set_{\st 1}=\Big\{\mxsqr, \{ N_{\st \prt}, \Delta_{\st \prt}, T_{\st \prt},  r_{\st \prt}, com_{\st \prt}, \vec{o}_{\st \prt}\}_{\st \forall \prt, 1\leq \prt \leq n}, \{K_{\st j}\}_{\st \forall \advb_{\st j}\in \corupt}
% %
% \Big\}$$
% 
%  where $\corupt$ is a set of corrupt parties, including server \srv.  
% 
% 
% \item by the end of the linear combination phase (before any puzzle is fully solved), it also learns:  
% %
% $$Set_{\st 2}=\Big\{ trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}, Y,  \{g_{\st 1}, \ldots, g_{\st \bar{t}}\}, \{com'_{\st \prt}, h_{\st \prt}, d_{\st 1, \prt},\ldots, d_{\st \bar{t}, \prt}   \}_{{ \st \forall \prt, 1\leq \prt \leq n}}, \{\bar f_{\st {\st l}}, \vv{ \gamma}'_{\st{l}}\}_{\st \forall\cl_{l}\in \{\corupt\cap\idx\}}\Big\}$$
% 
%  where $trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}$ is a set of messages sent to \srv during the execution of $\ole^{\st +}$. 
% \end{itemize}

We will argue that the probability that adversary  $\adv_{\st 2}\in\adv = (\adv_{\st 1}, \adv_{\st 2})$ outputs correct value of $b_{\st \prt}$ (in the experiment $\mathsf{Exp}_{\st \textnormal{prv}}^{\st\adv}(1^{\st\lambda}, n , \tl, t)$ defined in Definition \ref{def:privacy-vh-tlp}) is at most $\frac{1}{2}+\mu(\lambda)$. Since parameters $(\mxsqr, N_{\st \prt}, \Delta_{\st \prt}, T_{\st \prt}, Y, $ $ r_{\st \prt}, h_{\st \prt})$ have been picked independently of the plaintext messages/solutions, they reveal nothing about the messages. Each $y$-coordinate $\pi_{\st i, \prt}$ in $\vec{o}_{\st i, \prt}$ has been masked (or encrypted) with a fresh output of \prf (where ${o}_{\st i, \prt}\in \vec{o}_{\st \prt}$). Due to the security of  \prf, outputs of \prf are computationally indistinguishable from the outputs of a random function. As a result, a message blinded by an output \prf does not reveal anything about the message, except for the probability $\mu(\lambda)$. Also, each client $\prtt_{\st \prt}$ picks its secret keys and accordingly blinding factors independent of other clients. Therefore, knowing corrupt clients' secret keys $\{K_{\st j}\}_{\st \forall \advb_{\st j}\in \corupt}$ does not significantly increase the adversary's probability of winning the game in the experiment, given honest parties' puzzles and corresponding parameters. Because of the hiding property of the commitment scheme, commitments $com_{\st \prt}$ and $com'_{\st \prt}$ reveal no information about the committed value. 


Due to the security of $\ole^{\st +}$, a set $trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}$ of messages that \adv (acting on behalf of corrupt parties) receives during the execution of $\ole^{\st +}$ are (computationally) indistinguishable from an ideal model where the parties send their messages to a trusted party and receive the result. This means that the exchanged messages during the execution of $\ole^{\st +}$ reveal nothing about the parties' inputs, that include the encoded plaintext solution (i.e., $y$-coordinate $\pi_{\st i, \prt}$) and \prf's output used to encrypt $\pi_{\st i, \prt}$. 


Each $d_{\st i, \prt}$ is an output of $\ole^{\st +}$. Due to the security of $\ole^{\st +}$, it reveals to \adv nothing about the input of each honest client $\prtt_{\st \prt}$ to $\ole^{\st +}$, even if \srv inserts $0$. Moreover,  each $d_{\st i, \prt}$ has been encrypted with  $y_{\st i, \prt}$ which is a sum of fresh outputs of \prf. Recall that each $y_{\st i, \prt}$ has one of the following the forms:

\begin{itemize}[label=$\bullet$]

\item $y_{\st i, \prt}=  -\sum\limits_{\st \forall \cl_{_{\st l}}\in C\setminus\prtt_{\st\prt}}\prf(i, f_{\st {l}}) +  \sum\limits_{\st \forall \cl_{_{\st l}}\in \idx\setminus\prtt_{\st\prt}}\prf(i, \bar{f}_{\st {l}})      \bmod \prm$, when client $\prtt_{\st \prt}$ is one of the leaders, i.e., $\prtt_{\prt}\in \idx$. 

\item $y_{\st i, \prt}=    \sum\limits_{\st \forall \cl_{_{\st l}}\in\idx}\prf(i, \bar{f}_{\st {l}})         \bmod \prm$, when client $\prtt_{\st \prt}$ is not one of the leaders, i.e., $\prtt_{\st \prt}\notin \idx$. 

\end{itemize}

Due to the security of \prf, given secret keys $\{\bar f_{\st {\st l}}\}_{\st \forall\cl_{l}\in \{\mathcal{C}\cap\idx\}}$, it will be infeasible for \adv to learn anything about secret blinding factor used by each honest party, as long as the number of corrupt leaders is smaller than the threshold $t$, i.e., $|\corupt\cap \idx| < t$. Therefore,  given  $\{\bar f_{\st {\st l}}\}_{\st \forall\cl_{l}\in \{\mathcal{C}\cap\idx\}}$, \adv learns nothing about each honest client $\prtt_{\st \prt}$ $y$-coordinate $\pi_{\st i, \prt}$ (as well as $z'_{\st i, \prt}$ when $\prtt_{\st \prt}\in \idx$) in $d_{\st i, \prt}$, except with the negligible probability in $\lambda$, meaning that $d_{\st 1, \prt},\ldots, d_{\st \bar{t}, \prt}$ are computationally indistinguishable from random values, for $ \prt, 1\leq \prt\leq n$.  




Each puzzle $g_{\st i}$ that encodes a $y$-coordinate for the linear combination, uses the sum of $z'_{\st i, \prt}$ (and $w'_{\st i, \prt}$) to encrypt the $y$-coordinate, where each honest client's $z'_{\st i, \prt}$ is a fresh output of \prf and unknown to \adv.  Given corrupt clients' secret keys $\{K_{\st j}\}_{\st \forall \advb_{\st j}\in \corupt}$, \adv can remove the blinding factors $z'_{\st i, \prt}$ for the corrupt parties. However, due to the security of \prf and accordingly due to the indistinguishability of each $d_{\st i, \prt}$ from random values, it cannot remove $z'_{\st i, \prt}$ of honest parties from $g_{\st i}$ (before attempting to solve the puzzle) expect with the negligible probability in $\lambda$. 



Due to the security of \prf, given the encrypted $y$-coordinates of the roots $\{\vv{ \gamma}'_{\st{l}}\}_{\st \forall\cl_{l}\in \{\corupt\cap\idx\}}$ received by corrupt clients and the corrupt parties secret keys $\{K_{\st j}\}_{\st \forall \advb_{\st j}\in \corupt}$, \adv cannot learn the $y$-coordinates of the random root chosen by each honest client (accordingly it cannot learn the random root), except for a negligible probability in $\lambda$. 



%
%
%Each puzzle $g_{\st i}$ that encodes a y-coordinate for the linear combination, has also been encrypted with the sum of $z'_{\st i, \prt}$ (and $w'_{\st i, \prt}$), where each honest client's $z'_{\st i, \prt}$ is a fresh output of \prf and unknown to \adv.   Given corrupt clients' secret keys, \adv can remove the blinding factors for the corrupt parties, but, due to the security of \prf and the indistinguishability of each $d_{\st i, \prt}$, it cannot remove $z'_{\st i, \prt}$ of honest parties from $g_{\st i}$ (before solving the puzzle). 





%Due to the security of  \prf, each $g_{\st i}$ is computationally indistinguishable from a random value. 
%
Thus, given $Set_{\st 1}$ and $Set_{\st 2}$, if the sequential modular squaring assumption holds and factoring problem is hard, $\adv_{\st 2}$ that runs in time $\delta(T_{\st \prt})<T_{\st \prt}$ using at most $\bar{poly}(T_{\st \prt})$ parallel processors, cannot find a solution $m_{\st \prt}$  (from $\vec{o}_{\st \prt}$) significantly earlier than $\delta(\Delta_{\st \prt}$), except with negligible probability $\mu(\lambda)$. This means that it cannot output the correct value of $b_{\st \prt}$ (in the line \ref{expr-prv:puzzle-gen-state-guess} of experiment $\mathsf{Exp}_{\st \textnormal{prv}}^{\st\adv}(1^{\st\lambda}, n , \tl, t)$ defined in Definition \ref{def:privacy-vh-tlp}) with a probability significantly greater than $\frac{1}{2}$. 




Recall that each $d_{\st i, \prt}$ is blinded with a blinding factor $y_{\st i, \prt}$. These blinding factors will be cancelled out, if all $d_{\st i, \prt}$ (of different clients) are summed up. Given the above discussion, knowing the elements of $Set_{\st 1}$ and $Set_{\st 2}$, if the sequential modular squaring assumption holds and the factoring problem is hard, $\adv_{\st 2}$ that runs in time $\delta(Y)<Y$ using at most $\bar{poly}(Y)$ parallel processors, cannot output the correct value of $b_{\st \prt}$ (in the line \ref{expr-prv:adv-2-guess-again} of experiment $\mathsf{Exp}_{\st \textnormal{prv}}^{\st\adv}(1^{\st\lambda}, n , \tl, t)$ defined in Definition \ref{def:privacy-vh-tlp}) with a probability significantly greater than $\frac{1}{2}$. 


This means, \adv cannot find a solution
$\sum\limits_{\st \forall\prtt_{\st\prt}\in C}q_{\st \prt}\cdot m_{\st \prt}$ (from $g_{\st 1},\ldots, g_{\st \bar{t}}$) significantly earlier than $\delta(\Delta$), except with negligible probability $\mu(\lambda)$. Accordingly, \adv can only learn the linear \textit{combination of all honest clients' messages}, after solving puzzles $g_{\st 1},\ldots, g_{\st \hat{t}}$. 
%
\hfill$\blacksquare$
\end{proof}

We proceed to prove that \tf preserves a solution validity, w.r.t. Definition \ref{def:validity-vh-tlp}. 



\begin{lemma}\label{lemma:VH-TLP-solution-validity}
If the sequential modular squaring assumption holds, factoring $N$ is a hard problem, \prf is secure,  $\ole^{\st +}$ is secure (i.e., offers result validity and is privacy-preserving), and the commitment scheme meets the binding and hiding properties, then \tf preserves a solution validity, w.r.t. Definition \ref{def:validity-vh-tlp}. 
\end{lemma}
%


\begin{proof} We will demonstrate the probability that  a PPT adversary \adv  outputs an invalid solution but passes the verification (in the experiment $\mathsf{Exp}_{\st \textnormal{val}}^{\st\adv}(1^{\st\lambda}, n, \tl, t)$ defined in Definition 
\ref{def:validity-vh-tlp}) is negligible in the security parameter, i.e., $\mu(\lambda)$. 



In addition to $(Set_{\st 1}, Set_{\st 2})$, the messages that an adversary \adv receives  are as follows:

\begin{itemize}[label=$\bullet$]


\item by the end of  the puzzle-solving phase for a puzzle related to the linear combination, it learns: 
%
$$Set_{\st 3}=\Big\{\{root_{\st \prt}, tk_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\in \idx}, m=res    \Big\}$$

\item by the end of the puzzle-solving phase for a puzzle of a single honest client $\prtt_{\st \prt}$, it also learns:
%
$$Set_{\st 4}=\Big\{mk_{\st \prt}, m=m_{\st \prt} \Big\}$$
where \adv learns $Set_{\st 4}$ for any client (long) after it learns  $Set_{\st 3}$. 
\end{itemize}



Due to the binding property of the commitment scheme, the probability that \adv can open every commitment related to a valid root in $\{root_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\in \idx}$ to an invalid root (e.g., $root'$, where $root'\neq root_{\st \prt}$) and pass all the verifications, is  $(\mu(\lambda))^{\st |\idx|}$.
%due to the union bound, which is still negligible $\lambda$ (as $|\idx|$ has been set to be constant in $\lambda$). 
 Thus, this is detected in the step \ref{step-multi-client-verify-opening} of the protocol with a high probability, i.e., $1-(\mu(\lambda))^{\st |\idx|}$. 


As discussed in the proof of Lemma  \ref{lemma:VH-TLP-privacy}, before the puzzles of honest parties are solved, \adv learns nothing about the blinding factors of honest parties or their random roots (due to the hidden property of the commitment scheme, the privacy property of $\ole^{\st +}$, security of \prf, and under the assumptions that sequential modular squaring holds and factoring $N$ is a hard problem). 

Due to Theorem \ref{theorem::Unforgeable-Encrypted-Polynomial} (unforgeable encrypted polynomial with a hidden root), any modification by \adv to the inputs  $\{o_{\st 1, \prt}, \ldots, o_{\st \bar{t}, \prt}\}_{\st \forall \prtt_{\st \prt}\notin \corupt}$ and outputs $\{d_{\st 1, \prt}, \ldots, d_{\st \bar{t}, \prt}\}_{\st \forall \prtt_{\st \prt}\notin \corupt}$ of $\ole^{\st +}$, makes the resulting polynomial $\bm{\theta}$ not contain every root in $\{root_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\notin \corupt}$. The same applies to the generation of $\vec{g}=[g_{\st 1},\ldots, g_{\st \bar{t}}]$. Specifically, if each $g_{\st i}$ is not the sum of all honest parties $d_{\st i, \prt}$, then their blinding factors will not be cancelled out, making the resulting polynomial $\bm{\theta}$ not have every root in $\{root_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\notin \corupt}$, according to Theorem \ref{theorem::Unforgeable-Encrypted-Polynomial}. 
%
Thus, this can be detected with a high probability (i.e., at least $1-(\mu(\lambda))^{\st t}$) at step \ref{step-multi-client-check-roots} of the protocol.  



\adv will eventually learn the elements of $Set_{\st 3}$ for honest parties. However, this knowledge will not help it cheat without being detected, as \adv has already published the output of the evaluation, e.g.,  $\vec{g}=[g_{\st 1},\ldots, g_{\st \bar{t}}]$. 

Due to the security of $\ole^{\st +}$ (specifically result validity), any misbehaviour of \adv (corrupting \srv) during the execution of $\ole^{\st +}$ will not be detected only with a negligible probability $\mu(\lambda)$, in the steps \ref{eval:ole-detect} and \ref{eval:ole-detect-2} of the protocol. 

Hence, \adv cannot persuade \chal to return 1 on an invalid output of $\eval()$ (in the line \ref{expr-val:ver-2} of experiment $\mathsf{Exp}_{\st \textnormal{val}}^{\st\adv}(1^{\st\lambda}\, n  , \tl, t)$ defined in Definition \ref{def:validity-vh-tlp}) with a probability significantly greater than $\mu(\lambda)$. 


%=======. multiple invocations of Evaluate====
%\\
%
%Since  $\{root_{\st \prt}, tk_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\in \idx}\in Set_{\st 3}$ have been chosen uniformly at random for each instance of $\eval$, 
%
%==========\\


By solving a single client's puzzle (after all invocations of $\eval()$), \adv will also learn $Set_{\st 4}$ for each (honest) client $\prtt_{\st \prt}$.  Due to the binding property of the commitment scheme, the probability that \adv can open every commitment corresponding to the single message $m_{\st \prt}$ of each client $\prtt_{\st \prt}$ in $\{\prtt_{\st 1},\ldots, \prtt_{\st n}\}$ to an invalid message (e.g., $m'$, where $m'\neq m_{\st \prt}$) and pass the verification in the steps \ref{step-multi-client-check-single-puzzle-1} and \ref{step-multi-client-check-single-puzzle-2}  of the protocol is negligible, $\mu(\lambda)$. Note that the elements of set $\{root_{\st \prt}, tk_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\in \idx}\in Set_{\st 3}$ have been selected uniformly at random and independent of each solution  $m_{\st \prt}$. Thus, knowing elements $\{root_{\st \prt}, tk_{\st \prt}\}_{\st \forall \prtt_{\st \prt}\in \idx}$ will not increase the probability of the adversary to persuade a verifier to accept an invalid message $m'$, in the steps \ref{step-multi-client-check-single-puzzle-1} and \ref{step-multi-client-check-single-puzzle-2}  of the protocol. 


Thus, \adv cannot win and persuade \chal to return 1 on an invalid solution (in the line \ref{expr-val:ver-1} of experiment $\mathsf{Exp}_{\st \textnormal{val}}^{\st\adv}(1^{\st\lambda}, n, \tl, t)$) with a probability significantly greater than $\mu(\lambda)$. 
%
%Initially, we focus on the validity of a solution for a puzzle of a single client, $\prtt_{\st \prt}$. In this case, in addition to knowing $(Set_{\st 1}, Set_{\st 2})$, the adversary learns the puzzle's solution $(m_{\st \prt}, mk_{\st \prt})$ because it has already solved the puzzle. 
% you need to argue that proving the result of evaluation will not allow the adversary to cheat when it proves the solution for a single puzzle. 
\hfill$\blacksquare$\end{proof}


We have demonstrated that \tf is privacy-preserving (w.r.t. Definition \ref{def:privacy-vh-tlp})  and preserves solution validity (w.r.t. Definition \ref{def:validity-vh-tlp}). Hence, \tf is secure, according to Definition \ref{def:sec-def-vh-tlp}.  

This concludes the proof of Theorem \ref{theo:security-of-VH-TLP}.
%
\hfill$\square$\end{proof}












==> blank.tex <==
%!TEX root = main.tex



\section{Introduction}





==> cost-table-combined.tex <==
%!TEX root = main.tex








\begin{table*}[!htb]
%\begin{footnotesize}
\begin{center}
\caption{Complexities and features of  \mhtlp, \mmhtlp, and \tf intorduced in \cite{tempora-fusion}. In the figure, $n$ is the total number of clients, \tl is the number of leaders, $\cor=\tl+2$, 
$ \Delta$ is the period between granting the computation and when a linear combination of solutions is learned by server \srv, $\mxsqr$ is the maximum number of squarings that a solver can perform per second, $Y=\mxsqr\cdot \Delta$,  $z$ is the total number of puzzles given by a client to \srv, $\bar{\Delta}$ is the period between the discovery of two consecutive solutions. }
%
%
\label{complexity-of-our-schemes} 


\renewcommand{\arraystretch}{1.4}
\scalebox{0.66}{
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|c|c|} 
%\cline{1-9}
   \hline
   
   &&&&&&&\scriptsize Without&\multicolumn{2}{c|}{\scriptsize Supporting Verification}&\scriptsize Flexible&\\
   
   \cline{9-10}

   
 \multirow{-2}{*}{\scriptsize Schemes}&&\multirow{-2}{*}{\scriptsize Parties}&
\multirow{-2}{*}{\scriptsize Computation Cost}&\multirow{-2}{*}{\scriptsize Communication Cost}&\multirow{-2}{*}{\scriptsize Multi-Instance}&\multirow{-2}{*}{\scriptsize Multi-Client}&\multirow{-2}{*}{\scriptsize  Trusted-Setup}&{\scriptsize Client's Solution}&{\scriptsize Linear Combination}&\multirow{-2}{*}{\scriptsize Time Paramters}&\multirow{-2}{*}{\scriptsize Batch Solving}\\

\hline

        
        %%%%%%%%%
&&{\rotatebox[origin=c]{0}{\scriptsize }}\scriptsize Client&\cellcolor{gray!20} \scriptsize $O(z)$&\cellcolor{gray!20} \scriptsize $O(z)$&&&&&&& \\
 
      
        \cline{3-5}
   
   \multirow{-2}{*}{\rotatebox[origin=c]{20}{\scriptsize }}&&{\rotatebox[origin=c]{0}{\scriptsize  }} \scriptsize Verifier&\cellcolor{gray!20}\scriptsize $O(z)$&\cellcolor{gray!20}\scriptsize $-$&&&&&&&\\
  
   \cline{3-5}

  \multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \text{{\mhtlp}}}}&&{\rotatebox[origin=c]{0}{\scriptsize  }}\scriptsize Server&\cellcolor{gray!20}\scriptsize $O(z+Y+\mxsqr\cdot\sum\limits^{\st z}_{\st j=1}\bar{\Delta}_{\st j, \prt})$&\cellcolor{gray!20}\scriptsize $O(z)$&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize $\times$}}\\      
            
\hline

%%%%%

&&{\rotatebox[origin=c]{0}{\scriptsize }}\scriptsize Client&\cellcolor{gray!20} \scriptsize $O(\tl\cdot (z+n))$&\cellcolor{gray!20} \scriptsize $O((\tl+n)\cdot z)$&&&&&&& \\
 
      
        \cline{3-5}
   
   \multirow{-2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}&&{\rotatebox[origin=c]{0}{\scriptsize  }} \scriptsize Verifier&\cellcolor{gray!20}\scriptsize $O(\tl^{\st 2}+\tl+z)$&\cellcolor{gray!20}\scriptsize $-$&&&&&&&\\
  
   \cline{3-5}

  \multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \text{{\mmhtlp}}}}&&{\rotatebox[origin=c]{0}{\scriptsize  }}\scriptsize Server&\cellcolor{gray!20}\scriptsize $O(\tl\cdot (z+n+Y+\tl)+\mxsqr\cdot \sum\limits_{\st j=1}^{\st z}\bar{\Delta}_{\st j, \prt})$&\cellcolor{gray!20}\scriptsize $O(\tl\cdot n+z)$&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \checkmark}}&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize $\times$}}\\     

%%%%%
\hline
 
&& {\rotatebox[origin=c]{0}{\scriptsize }}\scriptsize Client&\cellcolor{gray!20} \scriptsize $O(\tl\cdot n)$&\cellcolor{gray!20} \scriptsize $O(\tl\cdot n)$&&&&&&& \\
 
      
      \cline{3-5}
   
 &&{\rotatebox[origin=c]{0}{\scriptsize  }} \scriptsize Verifier&\cellcolor{gray!20}\scriptsize $O(\tl^{\st 2}+\tl +z)$&\cellcolor{gray!20}\scriptsize $-$&&&&&&&\\
  
  \cline{3-5}

 \multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize  \cite{tempora-fusion}}}&&{\rotatebox[origin=c]{0}{\scriptsize  }}\scriptsize Server&\cellcolor{gray!20}\scriptsize $O(\tl\cdot (n+Y+\tl)+\mxsqr\cdot \sum\limits_{\st j=1}^{\st z}\Delta_{\st j, \prt})$&\cellcolor{gray!20}\scriptsize $O(\tl\cdot n)$&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize $\times$}}&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize $\times$}}\\
 
 

 %%%%%
\hline
 
&& {\rotatebox[origin=c]{0}{\scriptsize }}\scriptsize Client&\cellcolor{gray!20} \scriptsize $O(1)$&\cellcolor{gray!20} \scriptsize $O(1)$&&&&&&& \\
 
      
      \cline{3-5}
   
 &&{\rotatebox[origin=c]{0}{\scriptsize  }} \scriptsize Verifier&\cellcolor{gray!20}\scriptsize $-$&\cellcolor{gray!20}\scriptsize $-$&&&&&&&\\
  
  \cline{3-5}

 \multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize  \cite{MalavoltaT19}}}&&{\rotatebox[origin=c]{0}{\scriptsize  }}\scriptsize Server&\cellcolor{gray!20}\scriptsize $O(n+\mxsqr\cdot \sum\limits_{\st j=1}^{\st z}\Delta_{\st j, \prt})$&\cellcolor{gray!20}\scriptsize $O(1)$&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize $\times$}}&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}\\
 
 
 
   %%%%%
\hline
 
&& {\rotatebox[origin=c]{0}{\scriptsize }}\scriptsize Client&\cellcolor{gray!20} \scriptsize $O(1)$&\cellcolor{gray!20} \scriptsize $O(1)$&&&&&&& \\
 
      
      \cline{3-5}
   
 &&{\rotatebox[origin=c]{0}{\scriptsize  }} \scriptsize Verifier&\cellcolor{gray!20}\scriptsize $-$&\cellcolor{gray!20}\scriptsize $-$&&&&&&&\\
  
  \cline{3-5}

 \multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize  \cite{liu2022towards}}}&&{\rotatebox[origin=c]{0}{\scriptsize  }}\scriptsize Server&\cellcolor{gray!20}\scriptsize $O(n+\mxsqr\cdot(\frac{ \Delta}{\log(\mxsqr\cdot \Delta)}+ \sum\limits_{\st j=1}^{\st z}\Delta_{\st j, \prt}))$&\cellcolor{gray!20}\scriptsize $O(1)$&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize $\times$}}&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}} &\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}\\

 
 
    %%%%%
\hline
 
&& {\rotatebox[origin=c]{0}{\scriptsize }}\scriptsize Client&\cellcolor{gray!20} \scriptsize $O(1)$&\cellcolor{gray!20} \scriptsize $O(1)$&&&&&& &\\
 
      
      \cline{3-5}
   
 &&{\rotatebox[origin=c]{0}{\scriptsize  }} \scriptsize Verifier&\cellcolor{gray!20}\scriptsize $-$&\cellcolor{gray!20}\scriptsize $-$&&&&&&&\\
  
  \cline{3-5}

 \multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize  \cite{dujmovic2023time}}}&&{\rotatebox[origin=c]{0}{\scriptsize  }}\scriptsize Server&\cellcolor{gray!20}\scriptsize $O(n^{\st 2}+\mxsqr\cdot(\Delta+ \sum\limits_{\st j=1}^{\st z}\Delta_{\st j, \prt}))$&\cellcolor{gray!20}\scriptsize $O(1)$&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize $\times$}}&\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize \checkmark}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\times$}}&\multirow{-3}{*}{{\scriptsize $\checkmark$}}\\
 
 %%%%%%%%%%%%%%%%%
 

  
 \hline
 
 %%%%%%
 
 
 
\end{tabular}
}
\end{center}
%\end{footnotesize}
\end{table*}

==> literature-review.tex <==
% !TEX root =main.tex

%\subsection{Time-lock Puzzles}





\section{Related Work}\label{Related-Work}


==> old--solution-validity-def.tex <==
% !TEX root =main.tex


%%%%%%%%%%%%%%%%%%%%%%%%height=66mm,
{\small{
\begin{center}
\begin{mybox}[colback=white,  width=130mm,  left=-1mm, drop fuzzy shadow southwest]{$\mathsf{Exp}_{\st \textnormal{val}}^{\st\adv}(1^{\st\lambda}\text{, }n  \text{, } \tl \text{, } t)$}
$
  \begin{array}{l}
%
\setcounter{equation}{0}
\lnum \ssetup(1^{\st \lambda}, \tl, t)\rightarrow \kp_{\st \srv}:=(sk_{\st \srv}, pk_{\st \srv})\\
%
\lnum \mathsf{For}\;  \prt=1,\ldots, n\;\mathsf{do}: \\
%
%
\lnum\quad\csetup(1^{\st \lambda})\rightarrow \kp_{\st \prt}:=(sk_{\st \prt}, pk_{\st \prt})\\
%
%set variables
\lnum state\leftarrow \{pk_{\st \srv},  pk_{\st 1},\ldots, pk_{\st n}\}, \corupt\leftarrow \emptyset, \idx\leftarrow \emptyset\\
%
\lnum K\leftarrow \emptyset, cont\leftarrow True, counter\leftarrow 0, \vec{b}\leftarrow \bf{0}\\
%
\lnum \textnormal{For } 1,\ldots, \tl \textnormal{ do}: \\
%
\lnum \quad \textnormal{Select } a  \textnormal{ from}\ \{1,\ldots, n\}\\
%
\lnum \quad \idx \leftarrow \idx \cup\{\advb_{\st a}\}\\
%
\lnum\label{exp-val:start-while} \textnormal{While } (cont=True) \textnormal{ do}:\\
%
\lnum  \quad \adv(state, \opgen(), \oeval(), K, \idx, \Delta_{\st 1}, \ldots,  \Delta_{\st n}, \Delta, \mxsqr)\rightarrow (state, cont, \advb_{\st j})\\
%
%
\lnum  \quad \textnormal{If } cont =True, \textnormal{then}\\
%
\lnum \quad \quad  \corupt\leftarrow\corupt\  \cup\ \{\advb_{\st j}\}\\
%
\lnum\label{exp-val:end-while}  \quad \quad  K\leftarrow K_{\st \advb_{\st j}}\\
%
\lnum\label{expr-val:pick-messages}  \adv(state, K, \corupt, \opgen(), \oeval(), \corupt)\rightarrow \vec{m}=[m_{\st 1}, \ldots, m_{\st n}]\\
 %
% \mathsf{For}\ l=1,\ldots, |\corupt|\ \mathsf{do}: \\
 %

%
\lnum\label{expr-val:start-genPuz} \textnormal{For }  \prt=1,\ldots, n \textnormal{ do}: \\
%
\lnum\label{expr-val:endd-genPuz} \quad \pgen(m_{\prt}, \kp_{\st \prt}, pk_{\st \srv}, \Delta_{\st \prt}, \mxsqr)\rightarrow(\vec{o}_{\st \prt}, prm_{\st \prt})\\
%%%%%%%%%%%%%%
%\lnum \solv(., ., \vec{g}, \vec{pp}^{\st (\text{Evl})}, pk_{\st \srv}, \cmd)\rightarrow(m, .)\\

%%%%%%%%%%%%%
%\lnum \mathsf{For}\;  \prt=1,\ldots, n\;\mathsf{do}: \\
%
%




%%%%%%%%%%%%

 \lnum\label{expr-val:check-threshold} \textnormal{If } |\corupt\cap \idx|>t, \textnormal{then return } 0\\
 %
\lnum \label{expr-val:evaluate} \eval(\langle \hat{\srv}(\vec{o}, \Delta, \mxsqr, \vec{pp}, \vec{pk}, pk_{\st \srv}),  \hat{\prtt}_{\st 1}(\Delta, \mxsqr, \kp_{\st {\st 1}}, prm_{\st {\st 1}}, q_{\st 1}, pk_{\st \srv}), \ldots,  \hat{\prtt}_{\st n}(\Delta,\mxsqr,\\
%
\hspace{4.2mm} \kp_{\st {\st n}}, prm_{\st {\st n}}, q_{\st n}, pk_{\st \srv}) \rangle)\rightarrow(\vec{g}, \vec{pp}^{\st (\text{Evl})}), s.t.\\
%



 \lnum \label{expr-val:access-to-corrupt-server-keys} \quad  \textnormal{If } \hat{s}\in \corupt, \textnormal{then } \hat{s }  \textnormal{ has access to }  state   \textnormal{ and } K, \textnormal{else } \hat{\srv} \textnormal{ is an honest server, i.e., }  \hat{\srv} = \srv \\
 %
 \lnum \label{expr-val:access-to-corrupt-clients-keys}  \quad  \textnormal{If }  \hat{\prtt}_{\st j}\in \corupt, \textnormal{then}\ \hat{\prtt}_{\st j}\  \textnormal{has  access to} \ state\   \textnormal{and } K, \textnormal{else }  \hat{\prtt}_{\st j}\    \textnormal{is an honest client, i.e., } \hat{\prtt}_{\st j}=\prtt_{\st j}\\
%

\lnum\label{expr-val:solvPul-2} \solv(., ., \vec{g}, \vec{pp}^{\st (\text{Evl})}, pk_{\st \srv}, \ep)\rightarrow(m, \zeta)\\


%
\lnum\label{expr-val:reveal} \adv(state, K, \corupt, \orev(), m, \zeta, \vec{m},  \vec{o}_{\st 1}, \ldots, \vec{o}_{\st n},  \vec{pp}_{\st 1}, \ldots, \vec{pp}_{\st n}, \vec{g}, \vec{pp}^{\st (\text{Evl})})  \rightarrow  (m', \zeta') \\


\lnum \label{expr-val:ver-2}\textnormal{If } \ver(m', \zeta', .,., \vec{g},  \vec{pp}^{\st (\text{Evl})}, pk_{\st \srv}, \ep)\rightarrow 1, \text{s.t.}\   m'\notin \mathcal{L}_{\ep}, \textnormal{then return } 1 \\

\lnum\label{expr-val:start-solvePuz} \textnormal{For }  \prt=1,\ldots, n \textnormal{ do}: \\
%
\lnum\label{expr-val:end-solvPul} \quad \solv(\vec{o}_{\st \prt}, pp_{\st \prt}, ., ., pk_{\st \srv}, \scp)\rightarrow(\bar{m}_{\st \prt}, \zeta_{\st \prt})\\
%
\lnum\label{expr-val:guess-1}  \adv(state, K, \corupt, \opgen(), \oeval(), (\bar{m}_{\st 1}, \zeta_{\st 1}),\ldots,  (\bar{m}_{\st \prt}, \zeta_{\st \prt}), (m, \zeta),  \vec{m},  \vec{o}_{\st 1}, \ldots, \vec{o}_{\st n},  \\ 
 \hspace{4.2mm} \vec{pp}_{\st 1},\ldots, \vec{pp}_{\st n})  \rightarrow (m'_{\st \prt}, \zeta'_{\st \prt}, u)\\
%
\lnum\label{expr-val:ver-1}  \textnormal{If } %(K_{\st \advb_{\st \prt}} \notin K) \wedge
%
\ver(m'_{\st \prt}, \zeta'_{\st \prt}, \vec{o}_{\st \prt}, {pp}_{\st \prt}, .,., pk_{\st \srv}, \scp)\rightarrow 1, \text{s.t.}\   m'_{\st \prt}\notin \mathcal{L}_{\scp},   \textnormal{then return } 1\\
   \end{array} 
$
\end{mybox}
\end{center}
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






==> old-VH-TLP--proof.tex <==
%!TEX root = main.tex





\section{Proof of VH-TLP}\label{sec::VH-TLP-proof}

 
In this section, we prove the security of VH-TLP, i.e., Theorem \ref{theo:security-of-VH-TLP}. We initially prove that VH-TLP is privacy-preserving, w.r.t. Definition \ref{def:privacy-vh-tlp}. 

\begin{lemma}\label{lemma:VH-TLP-privacy}
If the sequential modular squaring assumption holds, factoring $N$ is a hard problem, \prf and $\ole^{\st +}$ are secure and the commitment scheme satisfies the hiding property, then VH-TLP is a privacy-preserving \vhtlp, w.r.t. Definition \ref{def:privacy-vh-tlp}. 

\end{lemma}

\begin{proof}
The messages that \srv receives are as follows.

\begin{itemize}[label=$\bullet$]
 \item by the end of puzzle generation phase, it learns: $Set_{\st 1}=\big\{\mxsqr, \{ N_{\st \prt}, \Delta_{\st \prt}, T_{\st \prt},  r_{\st \prt}, com_{\st \prt}, \vec{o}_{\st \prt}\}_{\st \forall \prt, 1\leq \prt \leq n}\big\}$. 
 
 
 \item by the end of the linear combination phase (before any puzzle is fully solved), it also learns:  
 $Set_{\st 2}=\big\{ trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}, Y,  \{g_{\st 1}, \ldots, g_{\st \bar{t}}\}, \{com'_{\st \prt}, h_{\st \prt}, d_{\st 1, \prt},\ldots, d_{\st \bar{t}, \prt}   \}_{{ \st \forall \prt, 1\leq \prt \leq n}}\big\}$, where $trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}$ is a set of messages sent to \srv during the execution of $\ole^{\st +}$. 
 \end{itemize}

We proceed to argue that the probability that adversary  $\adv = (\adv_{\st 1}, \adv_{\st 2})$ outputs correct value of $b$ (in the experiment defined in Definition \ref{def:privacy-vh-tlp}) is at most $\frac{1}{2}+\mu(\lambda)$. Since parameters $(\Delta_{\st \prt}, T_{\st \prt}, Y, r_{\st \prt}, h_{\st \prt})$ have been picked independently of the plaintext messages/solutions, they reveal nothing about the messages. Each $y$-coordinate in $\vec{o}_{\st \prt}$ has been masked (or encrypted) with a fresh output of \prf. Due to the security of  \prf, outputs of \prf are computationally indistinguishable from the outputs of a random function. As a result, a message blinded by an output \prf does not reveal anything about the message (except for the probability $\mu(\lambda)$). 


Because of the hiding property of the commitment scheme, commitments $com_{\st \prt}$ and $com'_{\st \prt}$ reveal no information about the committed value. Due to the security of $\ole^{\st +}$, a set $trans^{\ole^{\st +}_{\st \prt}}_{\st \srv}$ of messages that \se receives during the execution of $\ole^{\st +}$ are (computationally) indistinguishable from an ideal model where the parties send their messages to a trusted party and receive the result. This means that the exchanged messages during the execution of $\ole^{\st +}$ reveal nothing about the parties' inputs (that include the encoded plaintext solution and \prf's output used to encrypt the message). 


Each $d_{\st i, \prt}$ is an output of $\ole^{\st +}$. Due to the security of $\ole^{\st +}$, it reveals to \srv nothing about each $\prtt_{\st \prt}$'s input to $\ole^{\st +}$, even if \srv inserts $0$. Moreover,  
each $d_{\st i, \prt}$ has been encrypted with  $y_{\st i, \prt}$ which is a fresh output of \prf and unknown to \srv. Thus, $(d_{\st 1, \prt},\ldots, d_{\st \bar{t}, \prt})$ are computationally indistinguishable from random values, for $ \prt, 1\leq \prt\leq n$.  
%
Each $g_{\st i}$ has also been encrypted with $z'_{\st i, \prt}$ (and $w'_{\st i, \prt}$), where    $z'_{\st i, \prt}$ is a fresh output of \prf and and unknown to \srv.  Due to the security of  \prf, each $g_{\st i}$ is computationally indistinguishable from a random value. 
%
Thus, given $Set_{\st 1}$ and $Set_{\st 2}$, if the sequential modular squaring assumption holds and factoring problem is hard, $\adv_{\st 2}$ that runs in time $\delta(T_{\st \prt})<T_{\st \prt}$ using at most $\bar{poly}(T_{\st \prt})$ parallel processors, cannot find a solution $m_{\st \prt}$  (from $o_{\st \prt}$) significantly earlier than $\delta(\Delta_{\st \prt}$), except with negligible probability $\mu(\lambda)$. This means that it cannot output the correct value of $b$ (in the experiment defined in Definition \ref{def:privacy-vh-tlp}) with a probability significantly greater than $\frac{1}{2}$. 



Recall that each $d_{\st i, \prt}$ is blinded with a blinding factor $y_{\st i, \prt}$. These blinding factors will be cancelled out, if all $d_{\st i, \prt}$ (of different clients) are summed up. Thus, \srv can only learn the linear \textit{combination of all honest clients' messages} (after decrypting $g_{\st 1},\ldots, g_{\st \hat{t}}$). Hence, given $Set_{\st 1}$ and $Set_{\st 2}$, if the sequential modular squaring assumption holds and the factoring problem is hard, $\adv_{\st 2}$ that runs in time $\delta(Y)<Y$ using at most $\bar{poly}(Y)$ parallel processors, cannot find a solution
$\sum\limits_{\st \forall\prtt_{\st\prt}\in C}q_{\st \prt}\cdot m_{\st \prt}$ (from $g_{\st 1},\ldots, g_{\st \bar{t}}$) significantly earlier than $\delta(\Delta$), except with negligible probability $\mu(\lambda)$. This means that it cannot output the correct value of $b$ (in the experiment of Definition \ref{def:privacy-vh-tlp}) with a probability significantly greater than $\frac{1}{2}$. 
%
\hfill$\blacksquare$\end{proof}









==> old-privacy-def.tex <==
% !TEX root =main.tex




%%%%%%%%%%%%%%%%%%%%%%%%height=66mm,
{\small{
\begin{center}
\begin{mybox}[ colback=white,  width=130mm,  left=-1mm, drop fuzzy shadow southwest]{$\mathsf{Exp}_{\st \textnormal{prv}}^{\st\adv}(1^{\st\lambda}\text{, }n \text{, } \tl \text{, } t)$}
$
  \begin{array}{l}
%
\setcounter{equation}{0}
\lnum \ssetup(1^{\st \lambda}, \tl, t)\rightarrow \kp_{\st \srv}:=(sk_{\st \srv}, pk_{\st \srv})\\
%
\lnum \mathsf{For}\;  \prt=1,\ldots, n\;\mathsf{do}: \\
%
%
\lnum\quad\csetup(1^{\st \lambda})\rightarrow \kp_{\st \prt}:=(sk_{\st \prt}, pk_{\st \prt})\\
%
%set variables
\lnum state\leftarrow \{pk_{\st \srv},  pk_{\st 1},\ldots, pk_{\st n}\}, \corupt\leftarrow \emptyset, \idx\leftarrow \emptyset\\
%
\lnum K\leftarrow \emptyset, cont\leftarrow True, counter\leftarrow 0, \vec{b}\leftarrow \bf{0}\\
%
\lnum\label{expr-prv:start-pick-leaders} \textnormal{For } 1,\ldots, \tl \textnormal{ do}: \\
%
\lnum \quad \textnormal{Select } a  \textnormal{ from}\ \{1,\ldots, n\}\\
%
\lnum\label{expr-prv:end-pick-leaders} \quad \idx \leftarrow \idx \cup\{\advb_{\st a}\}\\
%
\lnum\label{expr-prv:start-corupt} \textnormal{While } (cont=True) \textnormal{ do}:\\
%
\lnum  \quad \adv_{\st 1}(state, \opgen(), \oeval(), K, \idx, \Delta_{\st 1}, \ldots,  \Delta_{\st n}, \Delta, \mxsqr)\rightarrow (state, cont, \advb_{\st j})\\
%
%
\lnum  \quad \textnormal{If } cont =True, \textnormal{then}\\
%
\lnum \quad \quad  \corupt\leftarrow\corupt\  \cup\ \{\advb_{\st j}\}\\
%
\lnum\label{expr-prv:end-corupt}  \quad \quad  K\leftarrow K_{\st \advb_{\st j}}\\
%

%
\lnum\label{expr-prv:pick-messages}  \adv_{\st 1}(state, K, \opgen(), \oeval(), \corupt)\rightarrow \vec{m}=[(m_{\st 0, 1}, m_{\st 1, 1}),\ldots, (m_{\st 0, n}, m_{\st 1, n})]\\
 %
% \mathsf{For}\ l=1,\ldots, |\corupt|\ \mathsf{do}: \\
 %

 %%%%%
%\lnum \textnormal{For every } \advb_{\st j} \in \corupt \textnormal{ do}: \\
% %
%\lnum  \quad \textnormal{If } j\in \idx, \textnormal{ then}\  counter\leftarrow counter+1\\
% %
%\lnum \textnormal{If } counter>t,\ \textnormal{then return } 0\\
%%%%%%
%
\lnum\label{expr-prv:puzzle-gen-start} \textnormal{For }  \prt=1,\ldots, n \textnormal{ do}: \\
%
\lnum \quad b_{\st \prt}\stackrel{\st \$}\leftarrow\{0, 1\}\\

\lnum \quad \vec{b}[\prt]\leftarrow b_{\st \prt}\\
%
\lnum\label{expr-prv:puzzle-gen-end}  \quad \pgen(m_{_{\st b_{\prt},\prt}}, \kp_{\st \prt}, pk_{\st \srv}, \Delta_{\st \prt}, \mxsqr)\rightarrow(\vec{o}_{\st \prt}, prm_{\st \prt})\\
%
\lnum\label{expr-prv:puzzle-gen-state} \adv_{\st 1}(state, K, \corupt,  \opgen(), \oeval(), \vec{o}_{\st 1}, \ldots, \vec{o}_{\st n},  \vec{pp}_{\st 1}, \ldots, \vec{pp}_{\st n})\rightarrow   state    \\ 
%
\lnum\label{expr-prv:puzzle-gen-state-guess} \adv_{\st 2}(\vec{o}_{\st 1}, \ldots, \vec{o}_{\st n},  \vec{pp}_{\st 1}, \ldots, \vec{pp}_{\st n},  state)\rightarrow (b'_{\st \prt}, \prt)\\
%
\lnum\label{expr-prv:chalenger-check-single-puzzle} \textnormal{If } (b'_{\st \prt}=\vec{b}[\prt]) \wedge (\advb_{\st \prt}\notin \corupt), \textnormal{then return } 1\\
%
 \lnum\label{expr-prv:check-threshold} \textnormal{If } |\corupt\cap \idx|>t, \textnormal{then return } 0\\
%
\lnum\label{expr-prv:evaluate} \eval(\langle \hat{\srv}(\vec{o}, \Delta, \mxsqr, \vec{pp}, \vec{pk}, pk_{\st \srv}),  \hat{\prtt}_{\st 1}(\Delta, \mxsqr, \kp_{\st {\st 1}}, prm_{\st {\st 1}}, q_{\st 1}, pk_{\st \srv}), \ldots,  \hat{\prtt}_{\st n}(\Delta,\mxsqr,\\
%
\hspace{4.2mm} \kp_{\st {\st n}}, prm_{\st {\st n}}, q_{\st n}, pk_{\st \srv}) \rangle)\rightarrow(\vec{g}, \vec{pp}^{\st (\text{Evl})}), s.t.\\
%
 \lnum\label{expr-prv:access-to-corrupt-server-keys} \quad  \textnormal{If } \hat{s}\in \corupt, \textnormal{then } \hat{s }  \textnormal{ has access to }  state   \textnormal{ and } K, \textnormal{else } \hat{\srv} \textnormal{ is an honest server, i.e., }  \hat{\srv}=\srv\\
 %
 \lnum\label{expr-prv:access-to-corrupt-clients-keys}   \quad  \textnormal{If }  \hat{\prtt}_{\st j}\in \corupt, \textnormal{then}\ \hat{\prtt}_{\st j}\  \textnormal{has  access to} \ state\   \textnormal{and } K, \textnormal{else }  \hat{\prtt}_{\st j}\    \textnormal{is an honest client, i.e., } \hat{\prtt}_{\st j}=\prtt_{\st j}\\
%
\lnum\label{expr-prv:reveal} \adv_{\st 1}(state, K, \orev(), \corupt, \vec{g}, \vec{pp}^{\st (\text{Evl})})\rightarrow   state    \\ 
%
\lnum\label{expr-prv:adv-2-guess-again} \adv_{\st 2}(\vec{o}, \vec{pp}, \vec{g}, \vec{pp}^{\st (\text{Evl})}, state)\rightarrow (b'_{\st \prt}, \prt)\\
%
\lnum\label{expr-prv:2nd-wining-condition} \textnormal{If } (b'_{\st \prt}=\vec{b}[\prt]) \wedge (\advb_{\st \prt}\notin \corupt), \textnormal{then return } 1,
\textnormal{else return }0
%
   \end{array} 
$
\end{mybox}
\end{center}
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






==> proof-of-correctness.tex <==
%!TEX root = main.tex



\section{Proof of Correctness}\label{sec::Proof-of-Correctness}


